Early Detection of Treatments Side Effect: A Sequential Approach

With the emergence and spread of infectious diseases with pandemic potential, such as COVID- 19, the urgency for vaccine development have led to unprecedented compressed and accelerated schedules that shortened the standard development timeline. In a relatively short time, the leading pharmaceutical companies1, received an Emergency Use Authorization (EUA) for vaccine\prime s en-mass deployment To monitor the potential side effect(s) of the vaccine during the (initial) vaccination campaign, we developed an optimal sequential test that allows for the early detection of potential side effect(s). This test employs a rule to stop the vaccination process once the observed number of side effect incidents exceeds a certain (pre-determined) threshold. The optimality of the proposed sequential test is justified when compared with the ({\alpha}, {\beta}) optimality of the non-randomized fixed-sample Uniformly Most Powerful (UMP) test. In the case of a single side effect, we study the properties of the sequential test and derive the exact expressions of the Average Sample Number (ASN) curve of the stopping time (and its variance) via the regularized incomplete beta function. Additionally, we derive the asymptotic distribution of the relative savings in ASN as compared to maximal sample size. Moreover, we construct the post-test parameter estimate and studied its sampling properties, including its asymptotic behavior under local-type alternatives. These limiting behavior results are the consistency and asymptotic normality of the post-test parameter estimator. We conclude the paper with a small simulation study illustrating the asymptotic performance of the point and interval estimation and provide a detailed example, based on COVID-19 side effect data (see Beatty et al. (2021)) of our suggested testing procedure.

==> fig2.tex <==
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[>=Latex,scale=0.3]
		\draw[help lines, color=gray!60](0,0) grid (20,15);
		\fill (0,0) node[left]{$O$} circle (.1);
		\draw[thick,->] (0,0) -- (22,0) node[anchor=north west]{$n$};
		\draw[thick,->] (0,0) -- (0,17) node[anchor=south west]{$S_n$};
		\draw[semithick, dashed,->] (0,0) -- (15,15);
		\draw (1,12) node[right]{stop and reject};
		\draw[semithick, dashed,->] (10,0) -- (20,10);
		\draw (15,3) node[right]{stop and accept};
		\draw[semithick,solid,->] (0,0) -- (1,0)-- (4,3)-- (5,3)-- (7,5)-- (8,5)-- (13,10);
		\draw (14,12) node[right]{continue};
		\fill (1,0)  circle (.1);
		\fill (2,1)  circle (.1);
		\fill (3,2)  circle (.1);
		\fill (4,3)  circle (.1);
		\fill (5,3)  circle (.1);
		\fill (6,4)  circle (.1);
		\fill (7,5)  circle (.1);
		\fill (8,5)  circle (.1);
		\fill (9,6)  circle (.1);
		\fill (10,7)  circle (.1);
		\fill (11,8)  circle (.1);
		\fill (12,9)  circle (.1);
	\end{tikzpicture}
	\label{sprt}
\end{figure}

==> fig3.tex <==
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[>=Latex,scale=0.3]
		\draw[help lines, color=gray!60](0,0) grid (20,15);
		\fill (0,0) node[left]{$O$} circle (.1);
		\draw[thick,->] (0,0) -- (22,0) node[anchor=north west]{$S_n^{x}$};
		\draw[thick,->] (0,0) -- (0,17) node[anchor=south west]{$S_n^{y}$};
		\fill (19,0) node[below]{$k^*_x+1$} circle (.2);
		\fill (19,1)  circle (.2);
		\fill (19,2)  circle (.2);
		\fill (19,3)  circle (.2);
		\fill (19,4)  circle (.2);
		\fill (19,5)  circle (.2);
		\fill (19,6)  circle (.2);
		\fill (19,7)  circle (.2);
		\fill (19,8)  circle (.2);
		\fill (19,9)  circle (.2);
		\fill (19,10) node[right]{$(k^*_x+1,k^*_y+1)$} circle (.2);
		\fill [color=brown](20,4) node[right]{-- not reject};
		\fill (20,6) node[right]{-- reject and stop vaccination};
		\fill (0,10) node[left]{$k^*_y+1$} circle (.2);
		\fill (1,10)  circle (.2);
		\fill (2,10)  circle (.2);
		\fill (3,10)  circle (.2);
		\fill (4,10)  circle (.2);
		\fill (5,10)  circle (.2);
		\fill (6,10)  circle (.2);
		\fill (7,10)  circle (.2);
		\fill (8,10)  circle (.2);
		\fill (9,10)  circle (.2);
		\fill (10,10)  circle (.2);
		\fill (11,10)  circle (.2);
		\fill (12,10)  circle (.2);
		\fill (13,10)  circle (.2);
		\fill (14,10)  circle (.2);
		\fill (15,10)  circle (.2);
		\fill (16,10)  circle (.2);
		\fill (17,10)  circle (.2);
		\fill (18,10)  circle (.2);
		\fill (19,10)  circle (.2);
		\draw[semithick,solid] (0,0) -- (1,1)-- (1,2)-- (2,3)-- (3,3)-- (4,4)-- (4,6)--(6,8)--(8,8)--(8,9)--(9,10);
		\fill (1,1)  circle (.1);
		\fill (1,2)  circle (.1);
		\fill (2,3)  circle (.1);
		\fill (3,3)  circle (.1);
		\fill (4,4)  circle (.1);
		\fill (4,5)  circle (.1);
		\fill (4,6)  circle (.1);
		\fill (5,7)  circle (.1);
		\fill (6,8)  circle (.1);
		\fill (7,8)  circle (.1);
		\fill (8,8)  circle (.1);
		\fill (8,9)  circle (.1);
		\draw[semithick,solid,color=brown] (0,0) -- (2,0)-- (4,2)-- (7,2)--(8,3)-- (10,3)-- (10,4)--(12,4);
        \fill [brown] (1,0)  circle (.1);
        \fill [brown](2,0)  circle (.1);
        \fill [brown](3,1)  circle (.1);
        \fill [brown](4,2)  circle (.1);
        \fill [brown](5,2)  circle (.1);
        \fill [brown](6,2)  circle (.1);
        \fill [brown](7,2)  circle (.1);
        \fill [brown](8,3)  circle (.1);
        \fill [brown](9,3)  circle (.1);
        \fill [brown](10,3)  circle (.1);
        \fill [brown](10,4)  circle (.1);
        \fill [brown](11,4)  circle (.1);
        \fill [brown](12,4)  circle (.2);
 
	\end{tikzpicture}
	\caption{The curtailed sequential test $\operatorname{T^*_{seq}}$}
\end{figure}


==> fig4.tex <==
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[>=Latex,scale=0.5]
		\draw[help lines, color=gray!60](0,0) grid (8,8);
		\fill (0,0) node[left]{$O$} circle (.1);
		\draw[thick,->] (0,0) -- (9,0) node[anchor=north west]{$S_n^{x}$};
		\draw[thick,->] (0,0) -- (0,9) node[anchor=south west]{$S_n^{y}$};
		\draw[semithick,solid,color=brown!60] (0,0) -- (1,1)-- (1,2)-- (2,3)-- (3,3)-- (4,4);
		\fill [color=brown](1,1)  circle (.1);
		\fill [color=brown](1,2)  circle (.1);
		\fill [color=brown](2,3)  circle (.1);
		\fill [color=brown](3,3)  circle (.1);
		\fill [color=brown!60](4,4) circle (.3 );

		\draw[thick,->,color=cyan] (4,4) -- (5,4) node[right,scale=0.8] {$p_{10}$};
		\draw[thick,->,color=cyan] (4,4) -- (4,5) node[above,scale=0.8] {$p_{01}$};
		\draw[thick,->,color=cyan] (4,4) -- (5,5)  node[right,scale=0.8] {$p_{11}$};
		\draw[thick,decoration={markings, mark=at position 0.3 with {\arrow{<}}},
		postaction={decorate},color=blue] (4,3.5) circle(0.5);
		\fill [color=blue](4,3) node[below,scale=0.8]{$p_{00}$} ;
		
		\fill (4,0) node[below,scale=0.8]{$i$} circle (.1);
		\fill (0,4) node[left,scale=0.8]{$j$} circle (.1);
		\fill (5,0) circle (.1);
		\fill (5.5,0) node[below,scale=0.8]{$i+1$}; 
		\fill (0,5) node[left,scale=0.8]{$j+1$} circle (.1);
	\end{tikzpicture}
\end{figure}
